Learning Shape Representations for Clothing Variations in Person Re-Identification

Person re-identification (re-ID) aims to recognize instances of the same person contained in multiple images taken across different cameras. Existing methods for re-ID tend to rely heavily on the assumption that both query and gallery images of the same person have the same clothing. Unfortunately, this assumption may not hold for datasets captured over long periods of time (e.g., weeks, months or years). To tackle the re-ID problem in the context of clothing changes, we propose a novel representation learning model which is able to generate a body shape feature representation without being affected by clothing color or patterns. We call our model the Color Agnostic Shape Extraction Network (CASE-Net). CASE-Net learns a representation of identity that depends only on body shape via adversarial learning and feature disentanglement. Due to the lack of large-scale re-ID datasets which contain clothing changes for the same person, we propose two synthetic datasets for evaluation. We create a rendered dataset SMPL-reID with different clothes patterns and a synthesized dataset Div-Market with different clothing color to simulate two types of clothing changes. The quantitative and qualitative results across 5 datasets (SMPL-reID, Div-Market, two benchmark re-ID datasets, a cross-modality re-ID dataset) confirm the robustness and superiority of our approach against several state-of-the-art approaches

==> exp/exp-MSMT17.tex <==
\begin{table*}[t]
  \scriptsize
  \caption{\textbf{Quantitative results of person re-ID on the MSMT17 dataset.} \emph{Left block}: standard re-ID evaluation. \emph{Right block}: extended re-ID setting. Note that all the reported results are reproduced using released codes available online. }
%   \vspace{-2.0mm}
  \centering
  \label{table:image-comparison}
  \resizebox{\linewidth}{!}
  {
  \begin{tabular}{l|cccc|cccc|cccc|cccc}
  %
  \toprule
  %
  \multirow{3}{*}{Method} & \multicolumn{4}{c|}{Standard re-ID evaluation} & \multicolumn{12}{c}{Extended re-ID evaluation}\\\cmidrule{2-17} 
  %
  & \multicolumn{4}{c|}{Query: RGB, Gallery: RGB}& \multicolumn{4}{c|}{Query: Gray, Gallery: RGB}& \multicolumn{4}{c|}{Query: RGB, Gallery: Gray}& \multicolumn{4}{c}{Query: Gray, Gallery: Gray}\\
  %
  & R1 & R5 & R10 & mAP & R1 & R5 & R10 & mAP & R1 & R5 & R10 & mAP & R1 & R5 & R10 & mAP\\
  %
  \midrule
  Verif-Identif [TOMM'17] & 60.7 & 76.0 & 80.1 & 31.4 & 12.6 & 21.9 & 26.7 & 5.7 & 20.0 & 34.4 & 42.0 & 7.3 & 31.2 & 46.0 & 52.9 & 10.9\\
  %
  SVDNet [ICCV'17] & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  Part-aligned~\cite{suh2018part} [ECCV'18] & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  FD-GAN~\cite{ge2018fd} [NIPS'18] & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  PCB~\cite{sun2018beyond} [ECCV'18] & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  DG-Net~\cite{zheng2019joint} [CVPR'19] & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  \midrule
  ResNet-50 (baseline) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  ResNet-50 (Gray Aug.) & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  Ours & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
  %
  \bottomrule
  %
  \end{tabular}
  }
\end{table*}
